Optimizing Vulnerability-Driven Honey Traffic Using Game Theory

Enterprises are increasingly concerned about adversaries that slowly and deliberately exploit resources over the course of months or even years. A key step in this kill chain is network reconnaissance, which has historically been active (e.g., network scans) and therefore detectable. However, new networking technology increases the possibility of passive network reconnaissance, which will be largely undetectable by defenders. In this paper, we propose Snaz, a technique that uses deceptively crafted honey traffic to confound the knowledge gained through passive network reconnaissance. We present a two-player non-zero-sum Stackelberg game model that characterizes how a defender should deploy honey traffic in the presence of an adversary who is aware of Snaz. In doing so, we demonstrate the existence of optimal defender strategies that will either dissuade an adversary from acting on the existence of real vulnerabilities observed within network traffic, or reveal the adversary's presence when it attempts to unknowingly attack an intrusion detection node.

==> subsections/framework.tex <==
\section{Framework}
\label{sec:Framework}
\ia{[Started editing this section]}
In this section we will discuss about the basic framework
\begin{figure}[htb]
  \centering
 \includegraphics[width=\linewidth]{images/scenario.png}
  \caption{Basic framework of \imph{Snaz}}
  \label{fig:framework}
\end{figure}


\subsection{Adversary}

As the discussion above, We assume the adversary already obtain one compromised OpenFlow switch at the beginning of the game. Via this compromised switch, attacker gathers information from the network flows as its belief. Meanwhile, the main goal of adversary is attack vulnerable hosts. 
In order to construct the attack, adversary capabilities include:
\begin{itemize}

\item Identify a flow $\langle o, d, i\rangle\in F$ that passes through the compromised switch, which $o$ and $d$ represent the source and destination IP address, and $i$ represents all the information inside packet.
\item Via $o, d$ and $i$, identify a vulnerability $v_t$ of a certain host $t$.
\end{itemize}

We represent attacker's belief as a tuple $\langle T, V\rangle$, which $T$ represents target set, and $V$ is vulnerabilities set. Each $t \in T$ represents one target asset, and $v_t \in V$ is defined as one vulnerability of target $t$. Through the passive scanning, attacker keeps updating the belief of suspect targets.

%$\langle l, t, v\rangle$, where $l\in C$ is the launching asset 
%\mps{switch or can it be an endpoint?---not too important}

%\mps{endpoint or can it be a switch?---important}}


%\paragraph{Attacker's moves:}

%\item A \emph{flow attack}, which seeks to compromise a target, is an attack on an existing flow (which could be a real flow or a honey flow). A flow attack is given by a tuple $\langle l, t, v\rangle$, where $l\in C$ is the launching asset \mps{switch or can it be an endpoint?---not too important}, $t$ is the target asset \mps{endpoint or can it be a switch?---important}, there is an endpoint $o$ and identifier $i$ such that $\langle o, t, i\rangle\in F$ is a flow, and $v\in V$ is the vulnerability of $t$ being attempted to be exploited.  

%\mps{In the above, an attacker can never compromise another switch it seems.}
%\mps{Also, the $v$ applies only to $t$ and not to $o$} 
%\whe{We should discuss this a little. Are we modifying a flow between two uncompromised endpoints in this attack? Or are we creating a new flow to attack a vulnerable endpoint? For the latter, we can (and should) spoof the source IP address, and as long as the reply traffic goes back through the attacker's switch, it can act as the endpoint with that IP address. Attacks could also come from compromised endpoints.}


\paragraph{Outcome of Attacker}
The outcome of a flow attack would be a compromise state, $C'$. If attackers trust the gathered information of a certain host, they can act on it to exploit further malicious actions.

\begin{itemize}

\item Success: the attacker applies the real vulnerabilities and gains control of the target. That is, $C' = C \cup \{t\}$ provided $v\in W_t$

\item Noop: the attacker's attempt fails and the asset remains uncompromised (but neither the attacker nor the defender's state changes in other respects). That is, $C' = C$ provided $v\not\in W_t$; the attacker acquires a belief that $v\not \in W_t$

\item Defeat: the attacker is detected and, as assumed, localized.  Thus the
attacker  loses control of the asset from which it launched the
attempt. That is, $C' = C \setminus \{l\}$ provided $\langle o, t, i\rangle\in H$
\end{itemize}


%\mps{Shall we separately consider a \emph{spoofing attack} in which the attacker produces a fake flow? There is no original flow and thus a honey flow won't be able to detect it. So out of our scope?}

%\paragraph{Initial condition:}
%Exactly one asset is compromised by the attacker ($|C| = 1$).

%\paragraph{Termination condition:}
%The attacker is removed ($C=\emptyset$) or the attacker accomplishes its mission ($C\cap G\neq\emptyset$).


\subsection{Defender}
To defend the passive scanning attack, defender can apply honey flow as deception. As discussed above, the background information of hosts can be used to identify the vulnerabilities by attackers. However, via honey flow, defender can delay the processes of reconnaissance or mislead attackers when they try to analysis packets headers for banner grabbing.
\paragraph{Honey Flow:}
About honey flow generation, we define $HF = \langle o, d, i\rangle$ for each honey flow, which:
\begin{itemize}
\item Origin $o$ and destination $d$ of the honey flow.

\item Other header information in the packets is $i$. From $i$, adversary can obtain one or more vulnerabilities, which is $i \rightarrow (V_h \subseteq V)$
%\item Generating packets that indicate $W_d = V_h$
\end{itemize}

%No change to the compromise state ensues, i.e., $C' = C$

%\item Fix an asset $n$. For a switch, reflash it, which causes no change to the topology. For an endpoint, apply a patch. Fixing is guaranteed to get rid of all \mps{for simplicity, all vulnerabilities and to clear out any compromise (if that asset is compromised).}
%\begin{itemize}
%\item $C' = C \setminus \{n\}$
%\item $W'_n = \emptyset$
%\end{itemize}


%We now consider about two kinds of misinformation that could offer to adversary.
%\begin{itemize}
%    \item Honey facts in data part: this misinformation include the honey username, password or URL. 
%    \item Honey facts in header part: this part can offer the misinformation about IP address, port situation and application background. 
%\end{itemize}

Besides, defender should not only consider how to confuse adversary, but also need to guarantee the availability of normal users, like avoiding congestion. For doing so, we apply $P_i$ as the number of packets passing through switch $i$, and $H_i$ is the number of honey packets go through the same switch at the same time. So $R_i=H_i/(P_i+H_i)$ is the honey traffic rate of switch $i$. 
$R_i$ can be used to evaluate the overhead of honey traffic, as well as the probability of misleading attackers. 


%We define honey flow as TCP based fake flow.It can transfer from one real host to a fake one or only transfer between two fake hosts. For doing so, defender need to generate and maintain fake IP addresses and port numbers as well as fake banner information. 

Figure 2 shows a scenario of defender and attacker movements. In this example, host 1 and host2 connect to each other with three OpenFlow switches (switch 1, switch 2 and switch 3) between them. Host 1 has vulnerability 1, which host 2 contains vulnerability 2. Switch 2 is compromised switch, and adversary has capability to scanning all traffic passing through switch 2. In order to protect hosts and disturb attacker reconnaissance processes, defender can deploy fake hosts(fake host 1 and 2) and create honey flows between them. Both of these two hosts can create TCP based honey flow and reveal any kind of fake vulnerability. For example, if these two hosts generate honey flow with vulnerability 1, attacker's belief includes four hosts information, and three of them own vulnerability 1.

\begin{figure}[htb]
  \centering
 \includegraphics[width=\linewidth]{scenario.png}
  \caption{Example of scenario}
  \label{fig:tags}
\end{figure}


\paragraph{Probabilistic representation:}
%\mps{\#2 Probabilities} Probabilities can apply to any part of the model but these are worth considering.

\begin{itemize}
%\item Weaknesses or distribution of vulnerabilities. \mps{Need to discuss. One way is to record the times when a vulnerability became known as well as the time of the last patching. Then $W_n$ = any vulnerabilities of the right age with prob 1.}

\item Initial value of C. $P(s\in C) = \frac{1}{|S|}$

\end{itemize}




There is one defender and one attacker and these are different parties.

\begin{itemize}
\item A finite set of assets (nodes), $N$, each of type \emph{endpoint} (e.g., host) $E$ or switch $S$, with at least two hosts and at least one switch. That is, $E\cap S=\emptyset$ and $E\cup S = N$.

%\item A topology is a relation, $T\subseteq N\times N$, where each host must connect to exactly one switch and a switch must connect to at least two other assets. \mps{not being used yet}

\item A defender's valuation is a function, $D: N\to \mb{R}$, specifying for each asset its valuation to the defender.  We may assume it is positive for the normal assets and zero for the honey assets---since the defender can discard any normal assets that are of zero or negative value. We write $D_n$ to refer to the defender's valuation of an asset $n$. 

\item An attacker's valuation is a function, $A: N\to \mb{R}$, specifying for each asset its valuation to the attacker.  This value may be negative since the attacker's mission may be damaged due to false information (for example).  We write $A_n$ to refer to the defender's valuation of an asset $n$. 

\item An attacker's goal is a set of endpoint assets, $G\subseteq E$, compromising \emph{any} of which would accomplish the attacker's mission. $G$ could be incorporated in $A$ but it is conceptually clearer to have it separate.

\item A nonempty, finite set of vulnerabilities, $V$.  Think of these as types or labels.

\item A network's weakness is a function, $W: N\to \wp(V)$. We write $W_n$ to refer to the weaknesses of an asset $n$. 

\item A network's compromise state, $C\subseteq N$, is the set of assets that have been compromised.

\item A flow is a tuple, $\langle o, d, i\rangle$ \mz{change to $\langle o, d, i, S\rangle$}, where $o, d\in E$ are endpoints (origin and destination, respectively) and $i\in\mb{N}$ is a natural number (flow identifier). $F\subseteq E\times E\times\mb{N}$ is the set of flows from the beginning of time till the end of time. Some flows may be inactive but that status is not relevant to this model.\mz{And $S$ is is a switch set which includes all the switches that the honey flow passes through.}

\item A network's honey state, $H\subseteq F$, is the set of honey flows.

\item 
\msm { A network's real state, $R\subseteq F$, is the set of real flows.}
\end{itemize}

==> subsections/oldexperiment.tex <==
\section{OLD EXPERIMENT}
\section{Game-Theoretic Experimental Evaluation}
\label{sec:Evaluation}

We evaluate our proposed Stackaleberg game model with different experiments and compare the results with two other defender's strategies (uniform random strategy and no-deception). In uni from random strategy, the defender generates honey flows randomly where in no-deception, he does not create honey flows at all.

Most of the experiments are conducted on a system with a 1.99 GHz Core-i7 CPU and 16.0 GB memory. The game model is solved by using linear programming where we have used CPLEX (version 12.8.0) solver to solve the programs.  
The parameters of the experiments are randomly generated, also, we run each experiment 100 times. 
The final results of the experiments are averaged for the generality. 
All random parameters are normalized to 1 except the numbers of \subsection{Optimal honey flow with fixed cost}
From the experiment analysis of game model, following conditions observed to get optimal Utility.
  
 The Analysis is true for any low cost between 0.001 to 0.1 and when the difference between different type of fake vulnerability hosts are not huge and ratio of no of hf/rf of different vulnerabilities are similar. if ratio of no of hf and no of rf for vulnerability V1 is 1 it works when ratio of no of hf and no of rf for vulnerability V2 is around 1 and less than 2.We are considering cost =0.1; 
\begin{Observation}{1}
\textbf{Observation 1}
\textbf{[When the fake host value is low and cost is fixed]}\item When fake host value is very low around one-third  of real host, defender’s utility will be optimal in following condition
\item  If number of honey flow implemented is 65 percent more than number of real flows.
\end{Observation}

\begin{Observation}{2}
\textbf{Observation 2}
\textbf{[When the fake host value is high and cost is fixed]}\item When fake host value is high around 85 percent of real vulnerability value or greater, defender’s utility will be optimal in following condition
\item  If number of honey flow implemented is 30 percent more than number of real flows

\end{Observation}
When fake host value is less than one-third of real vulnerability value defender's get his optimal utility when given honey flow is more than twice
By observing value of real vulnerability host and value of fake vulnerability host and the number of real flow our program can assign optimal honey flow.


The interpretation of our game model outcome for defender's utility with fixed cost is presented with following Algorithm.Which is based on the observations 1,2,3.The algorithm is with fixed cost in between 0.001 to 0.1 and the differences among different fake vulnerability values are not large. Ratio difference of no of honey flow and real flow of different type vulnerabilities are very close.
Important observation ratio of no of hf/rf of different vulnerability has to be close.  Such that if ratio of no of hf and no of rf for vulnerability V1 is 1 it works when ratio of no of hf and no of rf for V2 is around 1 and less than 2.
Below algorithm are considered based on the ratio of fake vulnerability values and real vulnerabilities values.Ratio greater than 0.85 interpret when fake vulnerability value is high, smaller than 0.3 interprets when fake vulnerability value is low .
\begin{algorithm}
\caption{Optimal honey flow algorithm}\label{alg:HF}
\begin{algorithmic}[1]
\Procedure{optimalhf}{rv[],fv[],numrf[]}%\Comment{The g.c.d. of a and b}
\State hf[]=[numrf.length]; 
\For{$i=0\ldots $numrf.length }%\Comment{We have the answer if r is 0}
\If{($fv[i]\geq0.85*rv[i]$ and $fv[i]\leq rv[i]$)}
   \State $hf[i]$$\approx$$0.3$*$numrf[i]+$numrf[i] \\
\ElsIf{($fv[i]\geq$0.5*$rv[i] and $fv[i]$<$0.85*rv[i])}
   \State $hf[i]\approx0.5*numrf[i]+numrf[i]$\\
\ElsIf{($fv[i]<0.5*rv[i]and $fv[i]$>$0.3*rv[i])}\\
   \State $hf[i]\approx0.65*numrf[i]+numrf[i]$\\
\State \textbf{else}
   \State $hf[i] \approx numrf[i]+numrf[i]$\\
   
\EndIf
%\textbf{End if}
\EndFor
%\textbf{End for}
\textbf{return hf[i]}
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{itemize}
    \item rv[]=array of real vulnerability value
    \item fv[]=array of fake vulnerability value
    \item numrf[]=array of number of real flow of each real vulnerability type
    \item hf[]=array of optimal honey flow (output)
\end{itemize}    

From the Algorithm It can be seen, if fake host value is too low implementing too many honey flow  might not be cost effective

\begin{Observation}{2}
\textbf{Observation 3}\\
\textbf{[Fake vulnerability value is around half of real value and cost is fixed]}\item When fake host value is half  real vulnerability value or greater, defender’s utility will be optimal in following condition
\item  Defender gets his optimal utility when honey flow is doubled than the real flow

\end{Observation}

\subsection{Visualizing solution impact of parameter}

\textbf{Graphical representation of observation 2 and Proof of algorithm analysis }

The following case a network setup consist of five different vulnerabilities and five different fake vulnerabilities values.Which follows Algorithm line 4 and 5
\begin{figure}[htb]
  \centering
\includegraphics[width=1.1\columnwidth,height=0.7\columnwidth]{images/hon1.png}
  \caption{Utility Vs HF/RF ratio}
  \label{fig:util}
\end{figure}
\begin{table}[!ht]
\centering\footnotesize\caption{Fake vulnerability is low and cost is fixed}
\begin{tabular}{lll}\hline
Real value&	fake value& no of real flow \\\hline
{10,20,30,40}&{9,18,27,32}& {5,5,5,5,5}\\
{10,20,30,40}&{9,18,27,32}& {10,10,10,10,10}\\\hline
\end{tabular}

\end{table}
These condition is also true for different number of honey flow of different type vulnerabilities.However the difference number of real flow from each type were not considered very high

\begin{table}[!ht]
\centering\footnotesize\caption{Defender's optimal utility with HF/RF ratio}

\begin{tabular}{llllll}\hline
hf/rf(rf10)& Ud&hf/rf(rf15)&	Ud&hf/rf(30)
\\\hline
{0.5}&{-4.6}&{0.5}&{-4.6}&{0.5}&	{-5.1}
\\ 
{1}&{-1.5}&{1}&{-2}&{1}&	{-3.5}\\
{1.2}&{-1.1}&{1.2}&{-1.6}&{1.2}&{-3.3}\\
{1.3}&{-1.1}&{1.4}&{-1.6}&{1.4}&{-3.3}\\
{1.6}&{-1.1}&{1.6}&{-1.6}&{1.6}&{-3.3}\\
{2}&{-1.1}&{2}&	{-1.6}&{2}&{-3.3}
\\\hline
\end{tabular}
%\source{Authors (In case defender utility does not change after HF/RF ration is greater than 1.3)}
\end{table}
 
\item As  fake  host  value  is  high  almost 90 percent of real vulnerability value or greater

\item Defender gets his optimal utility when honey flow is one-third more than the real flow.

Figure 2 shows when ratio of honey flow (HF) and real flow (RF) is 1.3 defender gets his optimal utility, analyzed for 5 different vulnerabilities 
hf/rf(rf10)= ratio of number of honey flow and number of real flow when number real flow is 10

\item\textbf{Graphical representation of observation 1 and Proof of algorithm analysis }\\
The  following  case  a  network  setup  consist  of  three different vulnerabilities and three different fake vulnerabilities values.\\

RV=Real Vulnerability set,FV=fake host set, rf(N)=number of real flow,
hf(N)=number of honey flow,Ud=Utility

\begin{table}[!ht]
\centering\footnotesize\caption{Fake vulnerability is high and cost is fixed}
\begin{tabular}{lllll}\hline
RV&FV& # rf(N) & hf(N)&Ud \\\hline
{10, 11,30}&{3, 4, 9}& {10, 20, 30}&{5,10,9}&-21.9\\
{10, 11,30}&{3, 4, 9}& {10, 20, 30}&{10,20,30}&-10.57\\
{10, 11,30}&{3, 4, 9}& {10, 20, 30}&{15,30,45}&-6.95
\\
{10, 11,30}&{3, 4, 9}& {10, 20, 30}&{17,34,50}&-6.13\\
{10, 11,30}&{3, 4, 9}& {10, 20, 30}&{20,40,50}&-6.13\\
\\\hline
\end{tabular}
\end{table}

Important observation ratio of no of hf/rf of different vulnerability has to be close. if ratio of no of hf and no of rf for V1 is 1 it works when ratio of no of hf and no of rf for V1 is around 1 and less than 2.
\begin{figure}[htb]
  \centering
\includegraphics[width=1.1\columnwidth,height=0.7\columnwidth]{images/vulnnew.png}
  \caption{Utility Vs HF/RF ratio}
  \label{fig:util}
\end{figure}
\item\textbf{ Relation between fake host value and Honey flow} 
\item Defender' can get optimal utility fast if fake value host and no of honey flow is high.
However those could be costly.Based on a real network with assigned value defender can find optimized value for both component. By changing
\begin{figure}[htb]
  \centering
 \includegraphics[width=\linewidth]{images/Op.png}
  \caption{Relation between fake vul and honey flow}
  \label{fig:util}
\end{figure}
Defender can get an optimal utility by applying high fake vulnerability value and low honey flow value or vice-versa also he can get an optimal value with by taking optimized value 
 \subsection{Impact of Honey Flow Cost}
 Our first experiment investigates the impact of cost associated with generating  honey flow in defender's utility. 
 We run this experiment with 5 types of vulnerabilities also.
 For Figure ~\ref{fig:flow-cost}, the number of real-flow is 500 and the honey flow are generated uniform randomly from [500,1000]. 
\begin{figure}[ht]
\includegraphics[width=1.0\columnwidth,height=1.1\columnwidth]{images/exp_1_cost_ab.png}
\centering
\caption{Comparison of defender utility when the defender uses different cost of generating an honey-flow a) the value of attacking a fake vulnerability is zero and a real is 1 \; b)  the value of attacking a fake vulnerability is exact same as real value and the values are randomly generate from[0.5, 1.0].}
\label{fig:flow-cost}
\end{figure}
 
 The results indicate that the Stackleberg model out performs than other models especially when the attacking penalty is high
 
 
\subsection{Deception with Unsophisticated Attackers }
In our previous experiments, we assumed that the attackers are always rational, but in the real world network scenarios, we can not always assume that the adversaries are all-time cautious. Thus, in this experiment investigates how the honey flow game models perform with the naive attackers. Here we consider two naive attackers ( Uniform Random and Greedy). 
In the uniform random model, the attacker's strategy is to attack all types of vulnerability uniformly where the defender's strategy is to generates optimal honey-flow against the attacker's strategy. 
On the other hand, in the greedy model, attacker calculates the expected payoffs for all types of vulnerabilities by considering the maximum honey-flow that the defender can generate for a type of vulnerability.  
Based on the calculation, he selects a vulnerability type to attack that gives him the maximum expected payoff. 
In both models, the attacker does not consider the defender's optimal strategies.

We also run this experiment with 5 types of vulnerabilities.
For Figure~\ref{fig:flow_ratio}, we investigate the defender utility when the defender sets a different upper bound of honey-flow compare to the real-flow numbers.
The number of real-flow is generated randomly from [500,1000], and the cost of a honey-flow is 0.0001 . 
We depict effect on defender's utility with different percent the honey-flows to the real-flows in this graph.

\begin{figure}[htb!]
\includegraphics[width=1.0\columnwidth,height=1.1\columnwidth]{images/exp_1_zero_vs_same.png}
\centering
\caption{Comparison of defender utility when a)  the value of attacking a fake vulnerability is exact same as real value  b) the value of attacking a fake vulnerability is zero and real one is 1.}
\label{fig:flow_ratio}
\end{figure}

The results show that creating fake flow provides significant defense against all mentioned attackers, especially when the attacker's choice is greedy but not rational. That is because the defender needs to create only that type of fake vulnerable flow in which the attacker is more biased

\subsection{ Scalability}
We evaluate the scalability of our LP solution. The results show in ~\ref{fig:time-complexity} where the game instances are randomly generated. For (b),  we set fix honey flow numbers. 
\begin{figure}[htb!]
\includegraphics[width=1.0\columnwidth,height=1.1\columnwidth]{images/exp_4_time_vul_ab.png}
\centering
\caption{Comparison of computational time when a)  the number of vulnerability is variable;  b)  the number of honey flow is variable}
\label{fig:time-complexity}
\end{figure}
The results show that the computational time grows exponentially either in increasing the number of vulnerabilities or the number of honey flows. However,  the graph of increasing vulnerability grows faster than the other one. That is because the best response constraints increase proportionally with the increasing number of vulnerabilities. 

\section{Mininet Testbed Evaluation}
\label{sec:Mininet}

To understand the applicability of above game model in real network scenario, we use the emulated environment of Mininet. The topology in Mininet follows figure 8. Other settings include:
\begin{figure}[htb!]
\includegraphics[width=1.0\columnwidth,height=0.5\columnwidth]{images/mininet.png}
\centering
\caption{Topology of Mininet Simulation}
\label{fig:mininet_topo}
\end{figure}
\begin{itemize}
    \item Client 1 connects with server 1, while client 2 connects with server 2.
    For simplification, in the simulation, both of these two clients send 500 packets based on TCP channel and receive replies.
    \item All the links in our simulation is 1 MBit/s bandwidth, 2ms delay and $2\%$ probability loss.
    \item The values of all the hosts are 1 and the cost to generate 1 honey flow is 0.0001. 
\end{itemize}
\begin{figure}[htb!]
\includegraphics[width=1.0\columnwidth,height=0.7\columnwidth]{images/one_vul.png}
\centering
\caption{Comparison of defender utility and attacker utility.}
\label{fig:cost_vul_2}
\end{figure}
In the first simulation, defender generates honey flow with fake vulnerability 1. The amount of honey flow increase from 1 to 500. The two fake clients send request and reply to each other and both of these two direction flows contain fake vulnerability 1.  Figure 8 shows the payoff of defender and attacker if attacker tries to deploy malicious actions based on vulnerability 1. The result shows that the payoff of attacker can be significant reduced if defender increase the ratio of honey flow.

Figure 10 shows the result when defender generate two kinds of fake vulnerabilities. In this simulation, the values of two clients are 2 and values of two servers are 1. Fake client 1 send request messages to fake client 2 with vulnerability 1 embedded, while the reply messages from fake client 2 to fake client 1 contain fake vulnerability 2.

\begin{figure}[htb!]
\includegraphics[width=1.0\columnwidth,height=0.7\columnwidth]{images/two_vul.png}
\centering
\caption{Comparison of defender utility and attacker utility.}
\label{fig:cost_vul_2}
\end{figure}
